Calorimeter-Based Triggers at the ATLAS Detector for Searches for Supersymmetry in Zero-Lepton Final States

This thesis consists of three closely related parts. An analysis of data recorded by the ATLAS detector in 2010 in proton-proton collisions at a center-of-mass energy of 7 TeV with an integrated luminosity of 33.4/pb is performed, searching for supersymmetric final states containing jets and missing transverse energy and no electrons or muons (zero-lepton channel). No excess over the Standard Model background expectation is observed. Using the CLs and PLR methods, exclusion limits are set in two different supergravity models. These considerably extend the excluded parameter ranges from earlier experiments. The rates and efficiencies of triggers based on combined signatures with jets plus missing transverse energy in ATLAS are studied, which are the primary triggers for the search for Supersymmetry in the zero-lepton channel. For the measurement of the efficiencies in data collected in 2010 and 2011, the bootstrap method is applied. Different sample triggers based on jets and missing transverse energy are compared and their efficiencies are measured. A reweighting approach is used to correct for the bias from the propagation of the uncertainties in the bootstrap method. A universal model is developed to describe the contribution of fake missing transverse energy from resolution effects to the rates of missing transverse energy triggers as function of the level of in-time pile-up, i.e. the number of concurrent proton-proton interactions. The input parameters are tuned to the properties of the ATLAS trigger system, and the model predictions are compared to measurements of trigger rates in ATLAS. Good agreement is found for low thresholds for which the rates are dominated by resolution effects, whereas the rates for higher thresholds are underestimated due to additional sources of fake and real missing transverse energy, which are not incorporated in the model.

==> Makefile <==
#
# (85)
#
# Makefile to compile Doktorarbeit and prepare Upload for arXiv.
#
# Note:
# * copied header.tex into doktor.tex
#
#


all: doktor.pdf

doktor.pdf:
	rm -f *bbl
	pdflatex doktor.tex
	makeindex doktor.idx
	bibtex doktor1
	bibtex doktor2
	pdflatex doktor.tex
	pdflatex doktor.tex
	pdflatex doktor.tex

localcopy:
	# remove bbl files, otherwise won't compile
	rm -f *bbl
	# create list of files used by latex (doktor.fls)
	pdflatex -recorder doktor.tex
	# copy all non-local files to local (outer loop not really necessary, could simply copy ALL files due 
	# to if [[ $$l == /* ]] statement
	for i in tex fd vf tfm cfg ldf def clo cls sty; do for l in `grep INPUT doktor.fls | grep "\.$$i" | uniq | awk '{print $$2}'`; do if [[ $$l == /* ]]; then echo $$l; cp $$l .;  fi;  done ; done
	# remove some files which are superfluous
	rm -f color.cfg  doktor.fls graphics.cfg  listings.cfg
	# doesn't work on arXiv with this file
	rm -f pdflatex.fmt
	# copy files *.bib to *.bib0 which don't get deleted after uploading to arXiv
	cp doktor_noweb.bib doktor_noweb.bib0
	cp doktor_web.bib doktor_web.bib0
	@echo "Run make clean now to remove remainders of processing (before packing and uploading)."

clean:
	# Don't remove *bbl and *ind because they are needed for arXiv upload
	@for i in log aux blg ilg loa lof out toc; do echo Removing '*'$$i ; find -iname '*'$$i'' | xargs rm -f ; done
	rm -f *~
	rm -f doktor.pdf
	rm -f doktor.dvi

.PHONY: doktor.pdf


==> bibtest.tex <==
%

%
%
\cite{ROOTUsersGuide}
\cite{URL_Alpgen}
\cite{URL_AthenaReleases}
\cite{URL_CaloCalib}
\cite{URL_COMA}
\cite{URL_CTEQ}
\cite{URL_DataLuminosity}
\cite{URL_ILCFacts}
\cite{URL_iLumiCalc}
\cite{URL_ISAJET}
\cite{URL_JetCleaning}
\cite{URL_JetMETRecommendation2010}
\cite{URL_Jimmy}
\cite{URL_LHCIncident}
\cite{URL_LHCUpgrade}
\cite{URL_LHeC}
%
\cite{URL_MSSMSquarkGluinoGRID}
\cite{URL_MSTW}
\cite{URL_mttwo}
\cite{URL_MuonRecoRel15}
\cite{URL_NIST1}
\cite{URL_nourldummy}
\cite{URL_Prospino}
\cite{URL_Pythia}
\cite{URL_Records}
\cite{URL_Reflex}
\cite{URL_SUSYxsec}
\cite{URL_TOPxsec}
\cite{URL_WTRPA}
%
\cite{Aitchison}
\cite{Barlow1989}
\cite{Binetruy}
\cite{CasellaBerger2001}
\cite{CINT}
\cite{Dehling2004}
\cite{Ellis1996}
\cite{Greiner3a}
\cite{Griffiths}
\cite{HalzenMartin}
\cite{Kleinknecht}
\cite{Langacker}
\cite{MartinShaw}
\cite{Maggiore}
\cite{Messiah2}
\cite{PeskinSchroeder}
\cite{Stock}
%
\cite{Abdus2011SUSYBenchmark}
\cite{Allanach2009}
\cite{Alner1987445}
\cite{Alpgen2003}
\cite{Amsler2008}
\cite{Athena2002}
\cite{ATLASDetector2008}
\cite{Baer2009}
\cite{BaerSUSYTools2009}
\cite{Bagnasco1994}
\cite{Barr2003}
\cite{Barr2009}
\cite{Beenakker1996}
\cite{Beenakker1997}
\cite{Beenakker1998}
\cite{Bennett2003}
\cite{Bisector1984}
\cite{Bhargava1981}
\cite{Cacciari2008}
\cite{Casadei2009}
\cite{CDFGluinosSquarks2002}
\cite{Chamseddine1982}
\cite{Cheng2002}
\cite{CMSHLT2006}
\cite{CMSLimits2010}
\cite{Combridge1977234}
\cite{CosmicRays2011}
\cite{Cowan2011}
\cite{Cowan2011PCL}
\cite{CRESST2011}
\cite{CSCNotes}
\cite{CTEQ6}
\cite{CTEQ6.6}
\cite{CTEQ6.6AS}
\cite{Degrassi2003}
\cite{Dijet2001}
\cite{Dimopoulos1995}
\cite{Doke2005}
\cite{DrellYan1970}
\cite{EventStreamingATLAS}
\cite{FEWZ2}
\cite{Gaudi2001}
\cite{Geant2003}
\cite{Gianotti2007}
\cite{Glashow1970}
\cite{Haag1975}
\cite{Hall1983}
\cite{Herwig2001}
\cite{Herwig2002}
\cite{HerwigSUSY2002}
\cite{Herwig++}
\cite{Herwig++23}
\cite{HLTSteering2008}
\cite{Isajet769}
\cite{Jimmy1996}
\cite{Junk1999}
\cite{Kidonakis2010}
\cite{KimNilles1984}
\cite{Kozanecki2009}
\cite{Langacker2003}
\cite{LangackerPolonsky1993}
\cite{LEPh02003}
\cite{Lester1999}
\cite{LHC_TDR_Published2008}
\cite{LHCf2011}
\cite{LuminosityEPJC}
\cite{MCatNLO2002}
\cite{MCatNLO2003}
\cite{MCatNLOSingleTop2006}
\cite{MCatNLOWtop2008}
\cite{Macesanu2006}
\cite{METPerformance2010}
\cite{Minuit1975}
\cite{Moneta2010}
\cite{MRSTLO2008}
\cite{MSTW2008}
\cite{Noether1918}
\cite{Olive2011}
\cite{PDB2010}
\cite{PLB2001AlephLimits}
\cite{PLB2004AlephLimits}
\cite{PLB2008D0Limits}
\cite{PLB2004L3Limits}
\cite{PLB2009D0Limits}
\cite{Polesello2010}
%
\cite{PRL101CDFLimits}
\cite{PRL102CDFLimit}
\cite{Pumplin2001}
\cite{PVReco2008}
\cite{Pythia6.4}
\cite{Quiros2006}
\cite{Read2002}
\cite{Read2002JoP}
\cite{ROOT1997}
\cite{Rubin1970}
\cite{Rubin1980}
\cite{Skands2004}
\cite{SNO2001}
\cite{SNO2005}
\cite{SUSYAnalyse0lepton2010}
\cite{SUSYPrimerMartin1997}
\cite{TechnicolorReview}
\cite{tHooft1971}
\cite{tHooft1973}
\cite{TopQuarkFBA_CDF2011}
\cite{TopQuarkFBA_LHC1}
\cite{TopQuarkFBA_LHC2011}
\cite{TopAntitopMass2011}
\cite{Tovey2008}
\cite{TriggerConfig2008}
\cite{TriggerPerf2010}
\cite{Wald1943}
\cite{Webber1999}
\cite{Wess1974}
\cite{Wilks1938}
\cite{WjetsD02011}
\cite{WmassTevatron2009}
\cite{WmassTevatronRev2008}
\cite{Zbjets2011}
\cite{Zwicky1933}
\cite{Zwicky1937}
%
\cite{ALEPH2002}
%
\cite{CMS-PAS-EGM-07-001}
\cite{LEPSUSYWG/01-03.1}
\cite{LEPSUSYWG/02-06.2}
\cite{LEPSUSYWG/04-01.1}
%
\cite{ATLASComputingTDR2005}
\cite{ATLASHLTTDR2003}
\cite{ATLASTDR1999}
\cite{CERN-LHCC-98-14}
\cite{LHC_TDR_CERN_Vol1}
\cite{LHC_TDR_CERN_Vol2}
\cite{LHC_TDR_CERN_Vol3}
\cite{TDRCalo1997}
%
\cite{ATL-COM-DAQ-2011-027}
\cite{ATL-COM-DAQ-2011-063}
\cite{ATL-COM-GEN-2007-003}
\cite{ATL-COM-GEN-2009-015}
\cite{ATL-COM-DAQ-2010-218}
\cite{ATL-COM-PHYS-2009-334}
%
%
\cite{ATL-COM-PHYS-2011-240}
\cite{ATL-DAQ-INT-2010-004}
\cite{ATL-DAQ-PROC-2010-017}
\cite{ATL-DAQ-PUB-2011-001}
\cite{ATL-LARG-PROC-2011-010}
\cite{ATL-LARG-PUB-2008-002}
\cite{ATL-PHYS-INT-2010-126}
\cite{ATL-PHYS-INT-2010-132}
\cite{ATL-PHYS-INT-2011-009}
\cite{ATL-PHYS-INT-2011-032}
\cite{ATL-PHYS-INT-2011-055}
\cite{ATL-PHYS-INT-2011-085}
\cite{ATL-PHYS-PROC-2009-113}
\cite{ATL-PHYS-PUB-2010-002}
%
\cite{ATLAS-CONF-2011-116}
\cite{ATLAS-COM-CONF-2011-195}
\cite{ATLAS-CONF-2010-005}
\cite{ATLAS-CONF-2010-024}
\cite{ATLAS-CONF-2010-027}
\cite{ATLAS-CONF-2010-038}
\cite{ATLAS-CONF-2010-039}
\cite{ATLAS-CONF-2010-053}
\cite{ATLAS-CONF-2010-054}
\cite{ATLAS-CONF-2010-056}
\cite{ATLAS-CONF-2010-057}
\cite{ATLAS-CONF-2010-060}
\cite{ATLAS-CONF-2010-064}
\cite{ATLAS-CONF-2011-007}
\cite{ATLAS-CONF-2011-011}
\cite{ATLAS-CONF-2011-021}
\cite{ATLAS-CONF-2011-032}
\cite{ATLAS-CONF-2011-046}
\cite{ATLAS-CONF-2011-063}
\cite{ATLAS-CONF-2011-101}
\cite{ATLAS-CONF-2011-106}
\cite{ATLAS-CONF-2011-116}
\cite{ATLAS-CONF-2011-132}
\cite{ATLAS-CONF-2011-135}
%
\cite{Hensel:1306492}
\cite{Maettig:1307100}
\cite{VanDerLeeuw2010}
\cite{Aracena:1303327}
%
\cite{JetCleaningPresentation2010}
\cite{URL_LHCIncident2}
%
%
%
%
%
%
%
%
%
%







==> chapters/nachspiel.tex <==
%

%
{
  \cleardoubleemptypage
  \thispagestyle{empty}
  SVN version: \texttt{$ $Id: nachspiel.tex 505 2012-02-28 00:18:35Z svn $ $}\\
  Compiled on \today\xspace at \currenttime.
  \newpage
}

%
{
  \cleardoubleemptypage
  \thispagestyle{empty}
  \vspace*{\fill}
  \begin{small}
  \centering
  The three graphical elements on the title page symbolize the three major projects documented in this thesis:
  %
  The left one is derived from
  %
  a comparison of predicted and observed rates for missing transverse energy triggers with different thresholds in 2010.
  The complete plot is shown in \Fig{fig:results_met_model_predictions_rates_2010}.
  %
  The one in the middle is derived from
  %
  %
  a two-dimensional turn-on curve of the combined \jetmet trigger \trigger{EF_j75_a4tc_EFFS_xe45_loose_noMu} obtained from the \tagname{Muons} stream.
  The complete plot is shown in \Fig{fig:results_trigger_performance_measurements_turnons_jetmet_muons_2d}.
  %
  The one to the right is derived from
  %
  exclusion limits as result of a search for Supersymmetry in zero-lepton final states, interpreted in a minimal supergravity model.
  A similar plot can be found in \Fig{fig:analysis_exclusion_limit_mSUGRA_CLs}.
  \end{small}
}


==> chapters/outlook.tex <==
%
%
%
%

%
%
%

